Adapting Personalized Speech Enhancement for Low-Latency Audio-Visual Target-Speaker Extraction

Online audio-visual target-speaker extraction aims to remove competing voices while preserving speech quality and bounding lookahead. Existing extractors are built and evaluated for separation on synthetic mixtures, leaving listening quality and meeting behavior largely untested. We introduce Audio-Visual Personalized Voice Quality Enhancement (AV-PVQE), which approaches these requirements from the other direction. We start from a personalized speech enhancement model that reconstructs a requested voice at high quality but confuses the target in 46% of two-speaker mixtures despite clean enrollment. Adding mouth features at its speaker-conditioning input and jointly fine-tuning the visual and reconstruction networks reduces this rate to 1.6%, with no future frames and 20 ms of algorithmic delay. Compared with an online autoregressive audio-visual extractor, AV-PVQE yields separation gains on two synthetic benchmarks and larger gains on recorded meetings, and keeps its advantage on excerpts with more speakers than the fine-tuning mixtures. In personalized P.835 listening tests on two meeting corpora, it improves overall quality over this extractor by 0.57 and 0.63 MOS, with similar mean rating relative to the starting model. Preservation and rejection tests show that it keeps the target intact when no competing voice is present and suppresses competing speech when the target is absent.

==> additional-human-results.tex <==
% Numerical source: author-supplied.tex, adopted at the user's direction on 2026-09-11.
% Scores and confidence intervals are supplied values; not independently recalculated.
% Source-only additional results. Not included in the main manuscript.
% Numerical provenance is the author's supplied revision, not the earlier report.
% These values/intervals were retained at the user's explicit direction after review.

\begin{table}[t]
\caption{Additional supplied V+E--PVQE differences on meetings. Each entry is V+E minus PVQE with its supplied 95\% confidence interval. Values were adopted at the author's direction on 11 September 2026 and were not independently recalculated.}
\label{tab:additional-pvqe}
\centering
\fontsize{9}{10.2}\selectfont
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}llr@{}}
\toprule
Dataset & Scale & \(\Delta\) vs PVQE [95\% CI]\\
\midrule
AMI & SIG & $-.11$ [$-.36$, .14]\\
 & BAK & +.08 [$-.10$, .26]\\
 & OVRL & $-.06$ [$-.24$, .12]\\
\midrule
MCoRec & SIG & +.24 [.00, .48]\\
 & BAK & +.10 [$-.08$, .28]\\
 & OVRL & +.17 [$-.01$, .35]\\
\bottomrule
\end{tabular}
\end{table}

\begin{table*}[t]
\caption{Additional supplied UniTalk human personalized P.835 results. Mean ratings are followed by V+E-minus-baseline differences and supplied 95\% confidence intervals. Values were adopted at the author's direction on 11 September 2026 and were not independently recalculated.}
\label{tab:additional-unitalk}
\centering
\fontsize{9}{10.2}\selectfont
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrr@{}}
\toprule
System / comparison & SIG & BAK & OVRL\\
\midrule
AVASE & 2.31 & 1.54 & 1.52\\
PVQE & \best{3.89} & \best{3.56} & \best{3.25}\\
V+E & 3.79 & 2.08 & 2.32\\
$\Delta$ vs AVASE & \best{+1.48 [1.22, 1.74]} & \best{+.54 [.36, .72]} & \best{+.80 [.62, .98]}\\
$\Delta$ vs PVQE & $-.10$ [$-.35$, .15] & \best{$-1.48$ [$-1.66$, $-1.30$]} & \best{$-.93$ [$-1.11$, $-.75$]}\\
\bottomrule
\end{tabular}
\end{table*}


==> architecture-compact.tex <==
% Optional native TikZ, one-column layout. Do not scale below natural size.
% Dependencies: tikz, amsmath, xcolor; \usetikzlibrary{arrows.meta}.
% Natural bounding box: 88 mm x 60 mm. All main labels are 9 pt; the fusion equation is 10 pt.
% The conditioning arrow ends at the PVQE boundary, without asserting an
% injection location among its inherited acoustic layers.
\begingroup%
\definecolor{vecaudio}{HTML}{176A70}%
\definecolor{vecvisual}{HTML}{654391}%
\definecolor{vecenroll}{HTML}{9A611F}%
\definecolor{vecink}{HTML}{26333A}%
\begin{tikzpicture}[
  x=1mm,y=1mm,>=Latex,
  font=\sffamily\fontsize{9}{10.3}\selectfont,
  text=vecink,inner sep=0pt,
  block/.style={draw,line width=.65pt,rounded corners=1.2pt,
    align=center,inner sep=1pt},
  signal/.style={-Latex,line width=.75pt,draw=vecink},
  visualsignal/.style={signal,draw=vecvisual},
  enrollsignal/.style={signal,draw=vecenroll}
]
\path[use as bounding box] (0,0) rectangle (88,60);

\node[align=center,text width=42mm] (mouth) at (22,58)
  {Target mouth video};
\node[align=center,text width=41mm] (enrollment) at (66.5,58)
  {Enrollment speech};

\node[block,draw=vecvisual,fill=vecvisual!7,
  minimum width=42mm,minimum height=12mm] (visual) at (22,48)
  {AV-HuBERT conv. encoder\\Current + 4 past frames};
\node[block,draw=vecenroll,fill=vecenroll!7,dashed,
  minimum width=41mm,minimum height=12mm] (speaker) at (66.5,48)
  {PVQE enrollment encoder\\Frozen};
\draw[visualsignal] (mouth.south) -- (visual.north);
\draw[enrollsignal] (enrollment.south) -- (speaker.north);

\node[block,draw=vecvisual,fill=vecvisual!7,
  minimum width=42mm,minimum height=8mm] (projection) at (22,34)
  {Projection $512\!\rightarrow\!176$};
\draw[visualsignal] (visual.south) -- (projection.north);

\node[block,draw=vecvisual,fill=vecvisual!3,
  minimum width=58mm,minimum height=12mm] (fusion) at (58,23) {};
\node[font=\sffamily\bfseries\fontsize{9}{10.3}\selectfont,
  text=vecvisual] at (58,26.9) {Gated fusion};
\node[font=\fontsize{10}{11.4}\selectfont] at (58,23)
  {$c_t=b_t+g_t\odot r(e)$};
\node at (58,19.2) {$r(e)$ starts at zero};
\draw[visualsignal] (projection.south) -- (22,26) -- (29,26);
\node[anchor=east,text=vecvisual] at (20.5,27) {$b_t$};
\draw[enrollsignal] (speaker.south) -- (66.5,29);
\node[anchor=west,text=vecenroll] at (68,35.5) {$e$ fixed};

\node[align=center,text width=17mm] (mix) at (9,22)
  {Mixture\\audio};
\draw[signal,draw=vecaudio] (mix.south) -- (9,12);

\draw[draw=vecaudio,line width=.8pt,rounded corners=1.5pt,
  fill=vecaudio!4] (1,.2) rectangle (71,12);
\node[font=\sffamily\bfseries\fontsize{9}{10.3}\selectfont,
  text=vecaudio] at (36,8.7) {Pretrained PVQE (fine-tuned)};
\node[align=center,text width=68mm] at (36,3.7)
  {STFT / encoder / recurrent / reconstruction};

\draw[visualsignal] (fusion.south) -- (58,12);
\node[anchor=east,text=vecvisual] at (56.5,14.5)
  {Conditioning input};
\node[align=center,text width=14mm] (output) at (81,6)
  {Target\\speech};
\draw[signal,draw=vecaudio] (71,6) -- (output.west);
\end{tikzpicture}%
\endgroup%


==> body.tex <==


\section{Video Enhanced model}
\subsection{Adapting the enhancement network}
Given a mixture $x[n]=s[n]+u[n]$, target video, and an enrollment speech recording, we estimate the target speech $s[n]$ while removing competing speech and other interference $u[n]$. We initialize the acoustic network from PVQE \cite{parnamaa2024personalized}. Its short-time Fourier transform (STFT), encoder, recurrent layers, and decoder reconstruct the waveform (Fig.~\ref{fig:architecture}). Its frozen enrollment encoder maps a separate target recording to a layer-normalized vector $e\in\mathbb{R}^{176}$, held fixed within each excerpt.

We add mouth features at the speaker-conditioning input using the convolutional encoder of AV-HuBERT \cite{shi2022avhubert}, and project its 512-dimensional features through two 256-dimensional hidden layers with rectified linear units to 176 dimensions. Following AVASE \cite{pan2025avase}, we repeat the visual features to match the audio feature rate. We denote the aligned cue by $b_t$.

The visual cue changes with articulation, whereas enrollment provides a fixed voice reference. We combine them through a gated enrollment residual:
\begin{equation}
\begin{aligned}
g_t&=\sigma\!\left(W_g[\bar b_t;e]+a_g\right),\\
r(e)&=W_2\operatorname{ReLU}(W_1e+a_1)+a_2,\\
c_t&=b_t+g_t\odot r(e),
\end{aligned}
\label{eq:fusion}
\end{equation}
where $\bar b_t=(t+1)^{-1}\sum_{j=0}^{t}b_j$ averages observed features from the excerpt's start, $\sigma$ is the sigmoid, and $\odot$ denotes elementwise multiplication. The enrollment projection has a 256-dimensional hidden layer. We initialize $W_2$ and $a_2$ to zero, so that adding enrollment initially gives $c_t=b_t$. We then learn the residual while fine-tuning the visual and reconstruction networks.

\subsection{Fine-tuning for online processing}
We train video conditioning, introduce the enrollment residual, and continue training on both corpora. For online operation, we replace whole-excerpt cue aggregation with the running mean in (\ref{eq:fusion}) and remap temporal decoder filters to current and past inputs, initializing newly introduced past taps to zero. We carry audio state across chunks and restrict visual encoding to the current mouth frame and its four predecessors. A final fine-tuning stage updates the visual path, fusion layers, and acoustic network together.

AV-PVQE has 12.79 million parameters and uses 16 kHz audio, a 20 ms STFT window, and a 10 ms hop. The visual input is 25 fps video with $88\!\times\!88$ grayscale mouth crops. AV-PVQE requires no future video, whereas RAVEN uses two future frames \cite{ma2025raven}. Changing future video left earlier visual outputs bit-exact; chunked and full-waveform audio outputs agreed above 128 dB SI-SNR. Device-level throughput and capture-to-output delay remain to be measured.

\input{table-extraction.tex}

\section{Experimental setup}
\subsection{Training data and model comparisons}
We generate two-speaker mixtures (2-spk-mix) from LRS3 and VoxCeleb2 following the mixing strategy used in prior work \cite{pan2025avase}. Each mixture combines two distinct speakers from the same corpus, with target-to-interferer SNRs within $[-10,10]$ dB. We use AVASE's recipe sizes of 40,000 training pairs and 5,000 fixed validation pairs, resampling training pairs and temporal excerpts each epoch. We extract each speaker in turn, using that speaker's video and a separate enrollment utterance.

We optimize with Adam at an initial learning rate of $10^{-3}$. The final stage runs for 30 epochs with batch size 16. We select the checkpoint using quieter-target validation mixtures, where the unmodified enhancer performs poorly. Test talks from LRS3 and test identities from VoxCeleb2 are excluded from fine-tuning. Each test uses 3,000 fixed pairs, with three-second LRS3 and four-second VoxCeleb2 excerpts.
% AUTHOR CHECK: recover final loss and schedule, training crop duration, and
% Adam implementation/settings. Only optimizer and initial LR are confirmed.

We reevaluate the released AVASE checkpoint with autoregressive inference and compare it with unmodified PVQE. All systems receive the same locally generated test mixtures; these scores are distinct from evaluations on AVASE's published test set. AVASE receives video without enrollment and derives its acoustic cue from previous output. AV-PVQE receives both video and enrollment, an additional source of target information; PVQE receives enrollment alone.

\input{table-speakers.tex}

\subsection{Meeting evaluation}
We test six-second excerpts from three meeting corpora without further fine-tuning. In the AMI Meeting Corpus \cite{carletta2005ami}, we sum participant headset channels to construct mixtures containing interference. The target headset provides an approximate reference because it contains crosstalk; enrollment uses a separate target interval. MTM contains four-participant Teams/Zoom meetings with separate participant channels and their exact sum. We evaluate target-present excerpts with ten-second target enrollment, grouping excerpts by the number of participants who speak anywhere within them.

MCoRec contains concurrent in-person conversations \cite{nguyen2025mcorec,mcorec2026data}. We use the central microphone as input. The target's worn microphone is not an exact reference contribution to that mixture, so we restrict evaluation to transcription, speaker similarity, and listening quality. Enrollment is PVQE-processed but remains imperfect. We conduct personalized listening tests on AMI and MCoRec.

\input{table-controls.tex}

\subsection{Objective measures and suppression tests}
We report scale-invariant signal-to-noise ratio improvement (SI-SNRi) relative to the input mixture \cite{leroux2019sdr}. We measure speaker similarity as the cosine similarity between Resemblyzer embeddings of output and target reference \cite{resemblyzer}; this evaluation encoder is independent of PVQE's enrollment encoder. Word accuracy (WAcc) is $100(1-\mathrm{WER})$, where WER counts word substitutions, deletions, and insertions. We transcribe outputs with Whisper \cite{radford2022whisper}. MCoRec uses corrected reference transcripts; the other corpora use Whisper transcripts of target references and thus measure transcription consistency. We report clip-median WAcc on synthetic tests and pooled word accuracy on meetings.

DNSMOS predicts speech quality (SIG), background quality (BAK), and overall quality (OVRL) from output audio \cite{reddy2022dnsmosp835}. We use the scorer's calibration for personalized enhancement consistently across corpora. We also report the DNSMOS P.808 overall estimate \cite{reddy2021dnsmos}. Both scorers receive output audio without enrollment.
% All SIG/BAK/OVRL values use the report's consistently calibrated pDNSMOS
% columns, labeled DNSMOS at the author's request. Identify scorer version
% and calibration in the reproducibility record; do not mix the two exports.

We test preservation by supplying target-only speech and the target cues supported by each system. We count target-speaker over-suppression (TSOS) events lasting more than one second: contiguous flagged frames with excessive loss of the target's compressed spectral magnitude \cite{eskimez2022personalized}. These events identify local speech loss that a whole-clip average can conceal. To measure changes in output level, we compute energy attenuation,
\begin{equation}
A=10\log_{10}\frac{\sum_n x[n]^2}{\sum_n\hat s[n]^2}.
\end{equation}
Unlike SI-SNR, this measure detects uniform gain loss. We report the fraction of target-only outputs with $|A|\leq3$ dB. This descriptive tolerance permits roughly half to twice the input energy; it is not a perceptual quality threshold.

When the target is absent, SI-SNR against the desired silent output is undefined. We therefore measure competing-speech energy attenuation, following PVQE's background-suppression evaluation \cite{parnamaa2024personalized}. We remove the target speaker's audio and repeat the least-motion frame from their video. AVASE and AV-PVQE receive the same static video, while AV-PVQE and PVQE retain target enrollment. This compares complete systems with different target cues.
% AUTHOR CHECK: recover TSOS compression exponent, threshold, frame settings,
% and event grouping from the scorer before submission.




\input{table-human.tex}

\subsection{Personalized listening study}
We use personalized ITU-T P.835 \cite{parnamaa2024personalized,naderi2021p835}. Listeners hear target enrollment, a one-second marker, and the processed excerpt without video, then rate SIG, BAK, and OVRL on five-point scales. We preserve output levels. Tasks contain 12 scored clips, four per system, plus trap and gold items.

An earlier LRS3 study gave an OVRL clip-difference standard deviation of 0.70 MOS. We used a planning standard deviation of 0.75 MOS to target a 0.15-MOS difference at two-sided $\alpha=0.05$ and 80\% power under an independent-pair normal approximation. We report corpus-specific, vote-weighted means and 95\% intervals using 50,000 bootstrap replicates that independently resample listeners and source cases.
% Full counts and conditional sample-size calculation are retained in the
% accompanying protocol record. This is not an achieved-power claim.
% Human means and intervals remain the author-supplied September 11 values.

% \newpage
\section{Results and discussion}
\subsection{Extraction and predicted quality}
The unmodified enhancer struggles most when the target is quieter than the interfering speaker. On quieter-target LRS3 mixtures, PVQE obtains $-7.38$ dB SI-SNRi, compared with 11.90 dB for AV-PVQE and 11.44 dB for AVASE. Across the complete synthetic tests, AV-PVQE improves SI-SNRi, word accuracy, and speaker similarity over AVASE (Table~\ref{tab:extraction}); the SI-SNRi gains are 0.31 dB on LRS3 and 1.84 dB on VoxCeleb2.



AV-PVQE also improves all four predicted-quality measures over AVASE. PVQE retains higher background and overall estimates despite its poorer target recovery; AV-PVQE has the highest predicted SIG on VoxCeleb2.

\subsection{Generalization to meetings}
The SI-SNRi gains over AVASE are larger on meetings: SI-SNRi increases by 4.43 dB on AMI and 6.58 dB on MTM, while WAcc rises from 50.14\% to 68.27\% and from 49.56\% to 67.65\%, respectively. AV-PVQE also has higher speaker similarity.

Although AV-PVQE is fine-tuned on two-speaker mixtures, it improves SI-SNRi over AVASE in all three MTM speaker-count groups (Table~\ref{tab:speakers}). Performance falls as more participants speak, with four-speaker SI-SNRi reaching 4.91 dB. On MCoRec, AV-PVQE raises WAcc from AVASE's 14.38\% to 25.38\% and speaker similarity from .824 to .838. Recognition remains difficult in these recordings despite the relative gain.


\subsection{Target preservation and rejection}
On target-only LRS3 speech, AV-PVQE produces seven long suppression events, compared with 142 for PVQE and none for AVASE (Table~\ref{tab:controls}). AV-PVQE's mean attenuation is closest to zero, but AVASE preserves level within $\pm3$ dB more often.

With competing-only speech and a static target image, AV-PVQE gives 32.83 dB mean attenuation, compared with 2.25 dB for AVASE and 2.46 dB for PVQE. Repeating a frame removes lip-motion evidence from both audiovisual systems; AV-PVQE still has enrollment, so the comparison is specific to these supplied cues. On naturally target-silent AMI excerpts, AV-PVQE's median attenuation is 7.25 dB. The controlled static-image result therefore does not establish reliable rejection during meetings.


\subsection{Listener-rated quality}
Listeners rate AV-PVQE above AVASE on SIG, BAK, and OVRL for both AMI and MCoRec (Table~\ref{tab:human}). All six AV-PVQE--AVASE difference intervals exclude zero. Overall gains are 0.57 MOS on AMI and 0.63 MOS on MCoRec.

\section{Conclusion}
We adapt a personalized enhancer for audiovisual target-speaker extraction without future video. AV-PVQE improves separation and transcription over AVASE on synthetic mixtures and meetings, with higher personalized listening ratings. Target-absent rejection remains incomplete. Matched audio-only and video-only controls are needed to isolate each cue's contribution. Future work includes device timing and joint enhancement/extraction training to retain noise, echo, and reverberation suppression.


==> figures/architecture.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{0.88\textwidth}{!}{%
  \begin{tikzpicture}[
      >=Latex,
      node distance=5mm and 7mm,
      block/.style={draw, rounded corners=1pt, align=center, inner sep=2.4pt,
                    font=\scriptsize},
      frozen/.style={block, dashed},
      signal/.style={font=\scriptsize, align=center}
    ]
    \node[signal] (video) {target mouth video\\frames $[t-4,t]$\\no future frame};
    \node[block, right=of video] (visual) {fine-tuned AV-HuBERT\\ResEncoder};
    \node[block, right=of visual] (projection) {$512\rightarrow256\rightarrow256
      \rightarrow176$\\projection + repeat/hold};

    \node[signal, below=9mm of video] (enroll) {disjoint clean\\enrollment};
    \node[frozen, right=of enroll] (pns) {frozen native PNS\\176-D identity};
    \node[block, right=of pns] (fusion) {cumulative visual gate\\+
      zero-initialized\\enrollment residual};

    \node[signal, below=9mm of enroll] (mix) {16 kHz\\mixture};
    \node[block, right=of mix] (stft) {causal STFT\\streaming state};
    \node[block, right=9mm of stft] (separator) {fully adapted\\causal separator};
    \node[signal, right=of separator] (out) {target\\estimate};

    \draw[->] (video) -- (visual);
    \draw[->] (visual) -- (projection);
    \draw[->] (projection) -- (fusion);
    \draw[->] (enroll) -- (pns);
    \draw[->] (pns) -- (fusion);
    \draw[->] (mix) -- (stft);
    \draw[->] (stft) -- (separator);
    \draw[->] (fusion) |- (separator);
    \draw[->] (separator) -- (out);
  \end{tikzpicture}}
  \caption{Streaming video-and-enrollment conditioning. The visual cue is the
  time-varying base. A gate computed from the observed visual prefix and
  normalized enrollment modulates a zero-initialized enrollment residual.
  Solid modules are adapted; the dashed enrollment encoder is frozen.}
  \label{fig:architecture}
\end{figure*}


==> figures/evaluation_map.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{0.96\textwidth}{!}{%
  \begin{tikzpicture}[
      >=Latex,
      node distance=4mm and 6mm,
      root/.style={draw, rounded corners=1pt, align=center, inner sep=3pt,
                   font=\scriptsize\bfseries},
      group/.style={draw, rounded corners=1pt, align=center, inner sep=3pt,
                    font=\scriptsize},
      metric/.style={draw, dashed, rounded corners=1pt, align=center,
                     inner sep=3pt, font=\scriptsize}
    ]
    \node[root] (query) {Desired output and\\reference role};

    \node[group, right=of query, yshift=18mm] (exact)
      {Exact target source\\LRS3, Vox2, AMI objective, MTM};
    \node[group, right=of query, yshift=6mm] (proxy)
      {Isolation-gated pseudo-reference\\natural AMI headset};
    \node[group, right=of query, yshift=-6mm] (mismatch)
      {Channel-mismatched target\\AMI far-field, MCoRec};
    \node[group, right=of query, yshift=-18mm] (none)
      {No target waveform/transcript\\UniTalk};
    \node[group, below=6mm of query] (zero)
      {Zero desired target\\absent/silent and secondary-only};

    \node[metric, right=12mm of exact] (mexact)
      {SI-SNRi, picked, STOIi,\\target cosine, transcript diagnostic};
    \node[metric, right=12mm of proxy] (mproxy)
      {Proxy intrusive scores, cosine,\\transcript, estimators, listening};
    \node[metric, right=12mm of mismatch] (mmismatch)
      {Identity/transcript diagnostics,\\estimators, listening};
    \node[metric, right=12mm of none] (mnone)
      {Enrollment cosine, estimators,\\listening};
    \node[metric, right=12mm of zero] (mzero)
      {ERLE/attenuation, output level,\\leakage and residual ASR};

    \draw[->] (query) -- (exact);
    \draw[->] (query) -- (proxy);
    \draw[->] (query) -- (mismatch);
    \draw[->] (query) -- (none);
    \draw[->] (query) -- (zero);
    \draw[->] (exact) -- (mexact);
    \draw[->] (proxy) -- (mproxy);
    \draw[->] (mismatch) -- (mmismatch);
    \draw[->] (none) -- (mnone);
    \draw[->] (zero) -- (mzero);
  \end{tikzpicture}}
  \caption{Evaluation is routed by the desired output and reference role.
  Intrusive metrics are not computed merely because a target-like channel is
  available. Human ratings and non-intrusive estimators remain separate from
  target-aware scores.}
  \label{fig:evaluation-map}
\end{figure*}


==> figures/fig_selection_bar.tex <==
% preamble: \usepackage{pgfplots} \pgfplotsset{compat=1.18}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar, bar width=8pt,
  width=\columnwidth, height=4.2cm,
  symbolic x coords={Quieter,Equal,Louder}, xtick=data,
  enlarge x limits=0.25,
  xlabel={Target level relative to competing speaker},
  ylabel={Target preference (\%)},
  ymin=0, ymax=100, ytick={0,25,50,75,100},
  ymajorgrids, grid style={gray!20},
  tick label style={font=\footnotesize},
  label style={font=\footnotesize},
  legend style={at={(0.5,1.03)}, anchor=south, legend columns=3,
                draw=none, font=\footnotesize,
                /tikz/every even column/.append style={column sep=6pt}},
]
\addplot[fill=orange!70, draw=none]
  coordinates {(Quieter,93.92) (Equal,98.58) (Louder,98.88)};
\addplot[fill=black!40, draw=none]
  coordinates {(Quieter,6.25) (Equal,61.08) (Louder,98.63)};
\addplot[fill=blue!60!black, draw=none]
  coordinates {(Quieter,97.00) (Equal,99.42) (Louder,99.25)};
\legend{AVASE, PVQE, AV-PVQE (ours)}
\end{axis}
\end{tikzpicture}
\vspace{-8pt}
\caption{Target preference on LRS3 by the target's level relative to the competing speaker. PVQE follows the louder voice; AV-PVQE selects the target at least 97\% of the time at every level.}
\label{fig:bylevel}
\vspace{-10pt}
\end{figure}
% \vspace{-10pt}

==> figures/fig_selection_levels.tex <==
% preamble: \usepackage{pgfplots} \pgfplotsset{compat=1.18}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  width=\columnwidth, height=4.2cm,
  symbolic x coords={Quieter,Equal,Louder}, xtick=data,
  enlarge x limits=0.15,
  xlabel={Target level relative to competing speaker},
  ylabel={Target preference (\%)},
  ymin=0, ymax=100, ytick={0,25,50,75,100},
  grid=major, grid style={gray!20},
  tick label style={font=\footnotesize},
  label style={font=\footnotesize},
  legend pos=south east,
  legend style={font=\footnotesize, draw=none, fill=none},
  mark size=2pt,
]
\addplot[thick, mark=triangle*, color=orange!80!black]
  coordinates {(Quieter,93.92) (Equal,98.58) (Louder,98.88)};
\addlegendentry{AVASE}
\addplot[thick, mark=square*, color=black!50]
  coordinates {(Quieter,6.25) (Equal,61.08) (Louder,98.63)};
\addlegendentry{PVQE}
\addplot[thick, mark=*, color=blue!70!black]
  coordinates {(Quieter,97.00) (Equal,99.42) (Louder,99.25)};
\addlegendentry{AV-PVQE (ours)}
\end{axis}
\end{tikzpicture}
\caption{Target preference on LRS3 by the target's level relative to the competing speaker. PVQE follows the louder voice; AV-PVQE selects the target at least 97\% of the time at every level.}
\label{fig:bylevel}
\end{figure}

==> implementation-details.tex <==
% Exact r6 equations retained for technical reference. Not included in the manuscript.
\begin{equation}
\begin{aligned}
 g_t &= \sigma\!\left(W_g[\bar b_t;e]+a_g\right),\\
 r(e)&=W_2\operatorname{ReLU}(W_1e+a_1)+a_2,\\
 c_t&=b_t+g_t\odot r(e).
\end{aligned}
\end{equation}

\begin{equation}
\mathrm{ERLE}=10\log_{10}\frac{\sum_n x[n]^2}{\sum_n\hat{s}[n]^2}.
\end{equation}


==> table-controls.tex <==
% All numerical cells follow the author's September 11 revision.
\begin{table*}[t]
\caption{LRS3 target preservation and response to a static target image. Long TSOS counts events lasting more than 1 s. Attenuation is averaged over clips: values near zero are preferable for target-only audio, and larger values for competing-only audio. Bold marks the best observed value.}
\label{tab:controls}
\centering
\fontsize{9}{10.2}\selectfont
\renewcommand{\arraystretch}{1.08}
\setlength{\tabcolsep}{5pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
 & \multicolumn{3}{c}{Target-only audio} & Competing-only audio\\
\cmidrule(lr){2-4}\cmidrule(l){5-5}
Model & Long TSOS\dn & Within $\pm3$ dB (\%)\up & Attenuation (dB) & Attenuation (dB)\up\\
\midrule
AVASE & \best{0} & \best{98.50} & .810 & 2.25\\
PVQE & 142 & 97.42 & .839 & 2.46\\
 VE & 7 & 96.93 & \best{.665} & \best{32.83}\\
\bottomrule
\end{tabular*}
\end{table*}


==> table-extraction.tex <==
% Existing cells follow author-supplied.tex; added DNSMOS cells
% follow the selected mixed-data, zero-future model in the manager report.
\begin{table*}[t]
\caption{Objective evaluation. Higher is better; bold marks the highest value per dataset and metric, without implying statistical significance. All entries are means except WAcc: clip medians on LRS3/VoxCeleb2 and pooled words on meetings. AMI SI-SNRi uses approximate headset references.}
\label{tab:extraction}
\centering
\fontsize{9}{10.2}\selectfont
\setlength{\tabcolsep}{4.4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrrrrrrr@{}}
\toprule
 & & \multicolumn{3}{c}{Target recovery} & \multicolumn{4}{c}{Predicted quality (DNSMOS)}\\
\cmidrule(lr){3-5}\cmidrule(l){6-9}
Dataset & Model & \shortstack{SI-SNRi\\(dB)\up} & \shortstack{WAcc\\(\%)\up} & Spk-sim\up & SIG\up & BAK\up & OVRL\up & P.808\up\\
\midrule
LRS3 & AVASE & 8.72 & 88.89 & .890 & 3.508 & 2.803 & 2.564 & 2.915\\
 & PVQE & $-2.31$ & 28.57 & .727 & \best{3.641} & \best{3.354} & \best{2.916} & \best{3.434}\\
 & \best{VE} & \best{9.03} & \best{90.91} & \best{.913} & 3.563 & 2.903 & 2.648 & 3.106\\
\addlinespace[2pt]
VoxCeleb2 & AVASE & 3.81 & 75.00 & .843 & 3.683 & 1.887 & 2.146 & 2.807\\
 & PVQE & $-2.97$ & 28.57 & .725 & 3.617 & \best{3.046} & \best{2.754} & \best{3.501}\\
 & \best{VE} & \best{5.65} & \best{82.35} & \best{.876} & \best{3.764} & 2.400 & 2.500 & 3.089\\
\midrule
AMI & AVASE & 2.56 & 50.14 & .864 & 2.593 & 3.879 & 2.195 & 2.858\\
 & PVQE & .40 & 18.51 & .851 & \best{3.226} & \best{4.311} & \best{2.893} & \best{3.451}\\
 & \best{VE} & \best{6.99} & \best{68.27} & \best{.885} & 2.947 & 3.967 & 2.481 & 3.065\\
\addlinespace[2pt]
MTM & AVASE & 3.06 & 49.56 & .867 & 2.781 & 3.571 & 2.352 & 3.034\\
 & PVQE & $-.08$ & 8.64 & .854 & \best{3.587} & \best{3.939} & \best{3.125} & \best{3.402}\\
 & \best{VE} & \best{9.64} & \best{67.65} & \best{.920} & 3.272 & 3.674 & 2.744 & 3.187\\
\bottomrule
\end{tabular*}
\end{table*}


==> table-human.tex <==
% Numerical source: author-supplied.tex, adopted at the user's direction on 2026-09-11.
% Scores and confidence intervals are supplied values; not independently recalculated.
\begin{table}[t]
\caption{Human personalized P.835 ratings (1--5), averaged over votes. The final column gives VE minus AVASE with its 95\% bootstrap confidence interval. Bold means are the highest for each scale.}
\label{tab:human}
\centering
\fontsize{9}{10.2}\selectfont
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Scale & AVASE & PVQE & VE & \shortstack{\(\Delta\) vs AVASE\\{[95\% CI]}}\\
\midrule
\multicolumn{5}{@{}l}{\textbf{AMI}}\\
SIG & 2.87 & \best{3.58} & 3.47 & \best{+.60 [.31, .90]}\\
BAK & 2.67 & 3.03 & \best{3.11} & \best{+.44 [.19, .69]}\\
OVRL & 2.11 & \best{2.74} & 2.68 & \best{+.57 [.32, .81]}\\
\midrule
\multicolumn{5}{@{}l}{\textbf{MCoRec}}\\
SIG & 1.65 & 2.39 & \best{2.63} & \best{+.98 [.74, 1.23]}\\
BAK & 1.28 & 1.84 & \best{1.94} & \best{+.66 [.49, .83]}\\
OVRL & 1.22 & 1.68 & \best{1.85} & \best{+.63 [.46, .80]}\\
\bottomrule
\end{tabular*}
\end{table}


==> table-speakers.tex <==
\begin{table}[t]
\caption{MTM separation by the number of participants who speak anywhere in an excerpt. Both models are evaluated on the same groups; VE is fine-tuned on two-speaker mixtures.}
\label{tab:speakers}
\centering
\fontsize{9}{10.2}\selectfont
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
 & \multicolumn{2}{c}{SI-SNRi (dB)\up}\\
Mixture group & AVASE & VE\\
\midrule
2-spk-mix & 4.27 & \best{12.16}\\
3-spk-mix & 1.92 & \best{7.13}\\
4-spk-mix & 0.65 & \best{4.91}\\
\bottomrule
\end{tabular}
\end{table}

